Critique on "Volume penalization for inhomogeneous Neumann boundary conditions modeling scalar flux in complicated geometry"

In this letter, we provide counter-examples to demonstrate that it is possible to retain second-order accuracy using Sakurai et al.'s method, even when different flux boundary conditions are imposed on multiple interfaces that do not conform to the Cartesian grid. We consider both continuous and discontinuous indicator functions in our test problems. Both indicator functions yield a similar convergence rate for the problems considered here. We also find that the order of accuracy results for some of the cases presented in Sakurai et al. are not reproducible. This is demonstrated by re-considering the same one- and two-dimensional Poisson problems solved in Sakurai et al. in this letter. The results shown in this letter demonstrate that the spatial order of accuracy of the flux-based VP approach of Sakurai et al. is between $\mathcal{O}$(1) and $\mathcal{O}$(2), and it depends on the underlying problem/model. The spatial order of accuracy cannot simply be deduced a priori based on the imposed flux values, shapes, or grid-conformity of the interfaces, as concluded in Sakurai et al. Further analysis is required to understand the spatial convergence rate of the flux-based VP method.

==> Software.tex <==
%The FD/BP algorithm and the numerical wave tank method described here is implemented within the IBAMR library~\cite{IBAMR-web-page}, which is an open-source 
%C++ simulation software focused on immersed boundary methods with adaptive mesh refinement;
%the code is publicly hosted at \url{https://github.com/IBAMR/IBAMR}.
%IBAMR relies on SAMRAI~\cite{HornungKohn02, samrai-web-page} for Cartesian grid management and the AMR framework. Linear and
%nonlinear solver support in IBAMR is provided by the PETSc library~\cite{petsc-efficient, petsc-user-ref, petsc-web-page}. All of the example cases
%in the present work made use of distributed-memory parallelism using the Message Passing Interface (MPI)
%library. 
%Simulations were carried out on both the XSEDE Comet cluster at the San Diego
%Supercomputer Center (SDSC) and the Fermi cluster at San Diego State University (SDSU).
%Comet houses 1,944 Intel Haswell standard compute nodes consisting of Intel Xeon 
%E5-2680v3 processors with a clock speed of 2.5 GHz, and 24 CPU cores per node.
%Fermi houses 45 compute nodes with different generations of Intel Xeon processors.  


%Between $64$ and $128$ cores were used for the 2D computations presented here, while $128$ cores were used for the 3D
%computations. The 2D ISWEC model using the medium grid resolution described in Sec.~\ref{subsec_grid_convergence}
%required approximately 6,129 seconds to execute 15,000 time-steps on Comet using $80$ cores. The 3D ISWEC model
%using the coarse grid resolution described in Sec.~\ref{subsec_3D_2D_models} required approximately 81,998 seconds
%to execute 10,000 time-steps on Fermi using $128$ cores of Intel Xeon E5-2697Av4 Broadwell processors with a clock speed of 2.6 GHz.
